TS2-Net: Token Shift and Selection Transformer for Text-Video Retrieval

Text-Video retrieval is a task of great practical value and has received increasing attention, among which learning spatial-temporal video representation is one of the research hotspots. The video encoders in the state-of-the-art video retrieval models usually directly adopt the pre-trained vision backbones with the network structure fixed, they therefore can not be further improved to produce the fine-grained spatial-temporal video representation. In this paper, we propose Token Shift and Selection Network (TS2-Net), a novel token shift and selection transformer architecture, which dynamically adjusts the token sequence and selects informative tokens in both temporal and spatial dimensions from input video samples. The token shift module temporally shifts the whole token features back-and-forth across adjacent frames, to preserve the complete token representation and capture subtle movements. Then the token selection module selects tokens that contribute most to local spatial semantics. Based on thorough experiments, the proposed TS2-Net achieves state-of-the-art performance on major text-video retrieval benchmarks, including new records on MSRVTT, VATEX, LSMDC, ActivityNet, and DiDeMo.

==> content/Introduction.tex <==
% 这里插入两张示意图：1张局部动作检索错误，1张局部物体检索错误。

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{pictures/intro_motivation.png}
    %\vspace{-0.8cm}
    \caption{Illustrator of our motivation. `Hat' is an tiny object that important for the final retrieval result and `Talking' is a slight action for final retrieval result. green: correct; red: incorrect}
    \label{fig:intro}
    \vspace{-0.5cm}
\end{figure*}

\section{Introduction}

Video Retrieval, which aims to retrieval relative video given a natural language, is a fundamental research task in visual-language understanding field. It has a number of potential applications in the fields of information retrieval, video recommendation, video-text generation and so on. In past years, several works are carried out \cite{bain2021frozen,chen2020fine,dzabraev2021mdmmt,gabeur2020multi,liu2019use,liu2021hit,luo2020univl} to solve this problem and make progress in public video-text benchmark\cite{anne2017localizing,xu2016msr,chen2011collecting,rohrbach2017movie,wang2019vatex,krishna2017dense}. 

% These works usually extract video features via off-line feature extractors, then train a module to aggregate these features.
% transformer 在视频领域展现了很大能力，现有的transformer architecture存在问题
The core of text-video retrieval is spatial-temporal feature modeling, which aims to learn representations of motions between video sequences and entities in video frames. Among a plethora of studies\cite{arnab2021vivit,liu2021video,bertasius2021space,bulat2021space} for spatial-temporal learning in videos, vision transformers have achieve superior performance on major benchmarks, while both the spatial and temporal representations are considered. 
Recent works \cite{bain2021frozen,luo2021clip4clip,fang2021clip2video,cheng2021improving} begin to train video-language model with raw video and text, using transformer architecture for video encoder.
Works like \cite{luo2021clip4clip,fang2021clip2video,cheng2021improving} decompose video encoder into two parts: per-frame extractor followed by a global feature aggregation, where spatial modeling and temporal modeling are individually. They lack fine-grained interaction between adjcant frames and only aggregate per-frame semantic information. 
%(Drawback: 缺少相邻帧之间的细粒度交互且最终得到的video embedding只是融合每帧的semantic information，比较粗糙).
Frozen\cite{bain2021frozen} employ divided space-time transformer in video encoder, and uses only one [CLS] token represent whole video feature. This architecture can learn large changing motion and categorical spatial semantics present on the whole video but still lack the capacity for tiny objects and movements. 

However, a video always contains richness semantic information (i.e. actions and objects) and we argue this compact video representation is not enough when it comes to slight movement and small objects.
For example, retrieving the ground truth from a video corpus in Fig.\ref{fig:intro} requires to notice the small object (`hat') and slight movement (`talking'). Based on structure of video transformer, video sequence is divided into continuous patches in space and time. In order to enhance the ability of modeling small object and slight movement, patch enhancement is an immediate thought. This motivates us to find a feasible method to incorporate spatial-temporal patch contexts into encoded features. 
In terms of temporal modeling, shift operation is introduced in TSM\cite{lin2019tsm}, which shift parts of the channel along temporal dimension. Shift ViT\cite{zhang2021token} apply shift in visual transformer to enhance temporal modeling. But transformer architecture is different from CNN architecture, and this partial shift strategy damages the completeness of each token representation.

% 他们这样的模型可以建模延续时间长的大动作和种类丰富的物体，但是对于局部的小动作和tiny object的识别不是很好。
% Nevertheless, these two representations on two different dimensions are complex enough to make it difficult to achieve both goals in the same network. 


% Commonly, spatiotemporal strengths are not equally likely. Large changing motion and categorical spatial semantics are present on the whole frame, while small movements and entities only exist on the local patch. These general spatial-temporal feature representations can be learned in the end-to-end approaches. However, fine-grained frame changes are difficult to capture. As shown in Fig1, the motion of xxx and object of xxx are ignored in the multi-modal interaction. 


% Based on structure of video transformer, video sequence is divided into continuous patches in space and time. In order to enhance the global and local model learning capacity simultaneously, patch enhancement is an immediate thought. This motivates us to find a feasible method to incorporate spatial-temporal patch contexts into encoded features.

In this paper, we present TS2-Net, a novel token shift and selection transformer network, to implement local patch feature enhancement. First, we adopt token shift module temporally shifts the whole spatial token features back-and-forth across adjacent frames, in order to capture local movement between frames. Second, we design a token selection module to select top-K informative tokens to enhance salient feature modeling capability. Our token shift module treats the features of each token as a whole, and iteratively swaps token features at the same location with neighbor frames, to preserve the complete local token representation. The token selection module estimates the importance of each token feature of patches with a selection network, which depends on the correlation between all spatial-temporal patch features and [CLS] tokens. Then it select tokens which contributes most to local spatial semantics. We align cross-modal representation in a fine-grained manner, where we calculate similarity with text and each frame-wise video embedding and aggregate them together. Specifically, TS2-Net is built on the common network structure of video-language contrastive learning.

We conduct extensive experiments on several video-text benchmarks, such as MSRVTT, VATEX, LSMDC, ActivityNet, and DiDeMo, to illustrate the effectiveness of our method. The experimental results demonstrate that
the proposed token shift and selection modules could improve the fine-grained text-video retrieval accuracy, and TS2-Net achieves SOTA performance on most of these datasets.  In summary, there are three main contributions in our paper:

\begin{enumerate}
    \item We put forward a new perspective of video-language learning with local patch enhancements, to improve the effect of fine-grained visual text retrieval, especially local actions and objects. 
    
    \item We introduce two modules, token shift and token selection, handling with local movements and local entities respectively, in both temporal and spatial manner. 
    
    \item We report new records of retrieval accuracy on several video-text retrieval benchmarks. Accompanied by thorough ablation studies, the large improvements are pin-pointed as contributions by our patch enhancement concept. 
\end{enumerate}

==> repeatcheet.tex <==
% \begin{table*}
% 	\begin{center}
% 	\caption{Text-to-Video retrieval results on VATEX and LSMDC. }
% 	\label{vatexlsmdc}
% % 		\resizebox{\textwidth}{!}{
% 			\begin{tabular}{c|ccccc|ccccc} % 控制表格的格式
% 	\hline
%     \multicolumn{3}{c}{}\multicolumn{4}{c}{VATEX} &\multicolumn{4}{c}{LSMDC} \\
%     \hline
% 	Method & R@1 & R@5 & R@10 & MdR & MeanR & R@1 & R@5 & R@10 & MdR & MeanR \\
%     \hline
%     % Random Baseline                               & 0.2  & 0.7  & 1.05    & 2000.5 & -   & 0.02 & 0.1 & 1.02 & 2100.5 & -\\
%     % VSE\cite{kiros2014unifying}                  & 28.0 & 64.3 & 76.9    & 3.0    & -   & -    &    - & -    &   -   & - \\
%     % VSE++\cite{faghri2017vse++}                  & 33.7 & 70.1 & 81.0    & 2.0    & -   & -    &    - & -    &   -   & - \\
%     JSFusion\cite{yu2018joint}                           & - & - & - & - & - & 9.1 & 21.2 & 34.1 & 36.0 & - \\
%     CE\cite{liu2019use}                           & - & - & - & - & - & 11.2 & 26.9 & 34.9 & 25.3 & - \\
%     MMT\cite{gabeur2020multi}                    & - & - & - & - & - & - & - & - & - & -\\
%     Dual Enc.\cite{dong2019dual}                 & 31.1 & 67.5 & 78.9    & 3.0    & -   & -    &    - & -    &   -   & - \\
%     HGR\cite{chen2020fine}                     & 35.1 & 73.5 & 83.5    & 2.0    & -   & -    &    - & -    &   -   & - \\
%     T2VLAD\cite{wang2021t2vlad}                  & - & - & - & - & - & 14.3 & 32.4 & 42.2 & 16 & -\\
%     CLIP\cite{radford2021learning}             & 39.7 & 72.3 & 82.2    & 2.0    & 12.8 & 11.3 & 22.7 & 29.2 &  -  & - \\
%     SUPPORT-SET\cite{patrick2020support}         & 44.9 & 82.1 & 89.7    & 1.0    & -   & - & - & -  & - & - \\
%     CLIP4Clip\cite{luo2021clip4clip}   & 55.9 & 89.2 & 95.0 & 1.0 & 3.9 & 22.6 & 41.0 & 49.1 & 11.0 & 61.0 \\
%     CLIP2Video\cite{fang2021clip2video}          & 57.3 & 90.0 & 95.5 & 1.0 & 3.6 & - & - & - & - & - \\
%     QB-Norm\cite{bogolin2021cross}                & 58.8 & 88.3 & 93.8 & 1.0 & - & 22.4 & 40.1 & 49.5 & 11.0 & -\\
%     CAMoE\cite{cheng2021improving}             & - & - & - & - & - & 22.5 & \textbf{42.6} & 50.9 & - & \textbf{56.5}\\
% 	\hline
% 	\textbf{Ours} & \textbf{59.1} & \textbf{90.0} & \textbf{95.2} & \textbf{1.0}  & \textbf{3.5} & {\bf 23.4}  & 42.3 &  {\bf 50.9} & \textbf{9.0} & 56.9\\
	
% 	\hline
% 		\end{tabular}%}
% 	\end{center}
% 		\vspace{-0.4cm}
% \end{table*}


% table begin
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{\textbf{The result on VATEX and LSMDC.}}
\label{table:fourbenchmarks}
\begin{tabular}{lccccccccc}
\hline\noalign{\smallskip}
\multirow{2}{*}{Model} & \multicolumn{4}{c}{VATEX} & & \multicolumn{4}{c}{LSMDC} \\[0.5pt]
\cline{2-5} \cline{7-10}
 & R@1 & R@5 & R@10 & MeanR & & R@1 & R@5 & R@10 & MeanR\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
T2VLAD\cite{wang2021t2vlad} & - & - & - & - &  & 14.3 & 32.4 & - & -\\
CLIP & 39.7 & 72.3 & 82.2 & 12.8 & & 11.3 & 22.7 & 29.2 & -\\
CLIP4Clip & 55.9 & 89.2 & 95.0 & 3.9 & & 21.6 & 41.8 & 49.8 & 58.0\\
CLIP2Video & 57.3 & 90.0 & \textbf{95.5} & 3.6 &   & - & - & - \\
QB-Norm & 58.8 & 88.3 & 93.8 & - & & 22.4 & 40.1 & 49.5 & -\\
CAMoE & - & - & - & - &  & 22.5 & {\bf 42.6} & 50.9 & 56.5\\
\textbf{Ours} & \textbf{59.1} & \textbf{90.0} & 95.2 & \textbf{3.5} & & {\bf 23.4}  & 42.3 &  {\bf 50.9} & 56.9\\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
% table end

% table begin
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{\textbf{The result on DiDeMo and ActivityNet-Caption.}}
\label{table:fourbenchmarks}
\begin{tabular}{lccccccccccc}
\hline\noalign{\smallskip}
\multirow{2}{*}{Model} & \multicolumn{4}{c}{ActivityNet} & & \multicolumn{4}{c}{DiDeMo} \\ 
\cline{2-5} \cline{7-10}
 & R@1 & R@5 & R@10 & MeanR & & R@1 & R@5 & R@10 & MeanR\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
T2VLAD\cite{wang2021t2vlad} & 23.7 & 55.5 & - & - & &\\
CLIP4Clip & 40.5 & 73.4 & - & 7.5 & & 43.4 & 70.2 & 80.6 & 17.5\\
QB-Norm & - & - & - & - & & 43.5 & 71.4 & 80.9 & -\\
Ours & {\bf 41.0} & {\bf 73.6} &  {\bf 84.5} & 8.6 & & 41.8 & {\bf 71.6} &  {\bf 82.0} & 14.8\\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
% table end


% table begin
\setlength{\tabcolsep}{2pt}
\begin{table}
\begin{center}
\caption{\textbf{The results on MSR-VTT-1kA.} Here DS means dual softmax mentioned in Section \ref{docu:dualsoftmax}.}
\label{table:msrvtt1k}
\begin{tabular}{c|ccccc|cccccc|}
\hline\noalign{\smallskip}
& & \multicolumn{5}{c}{Text \Longrightarrow Video} & \multicolumn{5}{c}{Video \Longrightarrow Text}\\
\hline
Model & R@1 & R@5 & R@10 & MdR & MeanR & R@1 & R@5 & R@10 & MdR & MeanR\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
% \multicolumn{}{l}{\textbf{\textit{Method without CLIP feature}}}\\
MMT \\
MDMMT \\
T2VLAD\cite{wang2021t2vlad}  & 29.5 & 59.0 & 70.1 & 4.0 & -\\
% \multicolumn{}{l}{\textbf{\textit{Method with CLIP(ViT-B/32)}}}\\
CLIP4Clip\cite{luo2021clip4clip}  & 44.5 & 71.4 & 81.6 & 2.0 & 15.3 & 42.7 & 70.9 & 80.6 & 2.0 & 11.6\\
CAMoE\cite{cheng2021improving}  & 44.6 & 72.6 & 81.8 & 2.0 & 13.3\\
LAFF\cite{hu2021lightweight}  & 45.8 & 71.5 & 82.0 & - & -\\
CLIP2Video\cite{fang2021clip2video}  & 45.6 & 72.6 & 81.7 & 2.0 & 14.6 & 43.5 & 72.3 & 82.1 & 2.0 & 10.2\\
\textbf{Ours}  & {\bf 47.0}  & {\bf 74.5} & {\bf 83.8} & {\bf 2.0} & {\bf 13.0} & {\bf 45.3} & {\bf 74.1} & {\bf 83.7} & {\bf 2.0} & {\bf 9.2}\\
CLIP2Video\cite{fang2021clip2video}  & 48.6 & 75.4 & 84.4 & 2.0 & 11.9\\
CAMoE\cite{cheng2021improving}  & 47.3 & 74.2 & 84.5 & 2.0 & 11.9\\
\textbf{Ours} & {\bf 51.1}  & {\bf 76.9} &  {\bf 85.6} & {\bf 1.0} & {\bf 11.7}\\
\hline
% \multicolumn{}{l}{\textbf{\textit{Method with CLIP(ViT-B/16)}}}\\
CLIP2TV\cite{gao2021clip2tv} & 48.3 & 74.6 & 82.8 & 2.0 & 14.9\\
\textbf{Ours} & {\bf 49.4}  & {\bf 75.6} &  {\bf 85.3} & {\bf 2.0} & {\bf 13.5} & {\bf 46.6}  & {\bf 75.9} &  {\bf 84.9} & {\bf 2.0} & {\bf 8.9}\\
CLIP2TV\cite{gao2021clip2tv} & 52.9 & 78.5 & 86.5 & 1.0 & 12.8\\
\textbf{Ours} & {\bf 54.0}  & {\bf 79.3} &  {\bf 87.4} & {\bf 1.0} & {\bf 11.7}\\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
% table end


% table begin
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{The results on VATEX}
\label{table:vatex}
\begin{tabular}{lcccc}
\hline\noalign{\smallskip}
\multirow{2}{*}{Model} & \multicolumn{4}{c}{VATEX} \\ \cline{2-5}
 & R1 & R5 & R10 & MeanR\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
CLIP & 39.7 & 72.3 & 82.2 & 12.8\\
CLIP4Clip & 55.9 & 89.2 & 95.0 & 3.9\\
CLIP2Video & 57.3 & 90.0 & 95.5 & 3.6\\
QB-Norm & 58.8 & 88.3 & 93.8 & -\\
LAFF* & 59.1 & {\bf 91.7 } & {\bf 96.3} & -\\
Ours & {\bf 60.0}  & 89.8 &  95.1 & {\bf 3.5}\\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
% table end

\textbf{LSMDC}Results are given in Table~\ref{table:lsmdc}.

% table begin
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{The results on LSMDC}
\label{table:lsmdc}
\begin{tabular}{lcccc}
\hline\noalign{\smallskip}
Model & R1 & R5 & R10 & MeanR\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
CLIP & 11.3 & 22.7 & 29.2 & -\\
CLIP4Clip & 21.6 & 41.8 & 49.8 & 58.0\\
QB-Norm & 22.4 & 40.1 & 49.5 & -\\
CAMoE & 22.5 & {\bf 42.6} & 50.9 & 56.5\\
Ours & {\bf 23.4}  & 42.3 &  {\bf 50.9} & 56.9\\
Ours(dsl) & 22.4 & 44.1 & 52.5 & 55.6\\
CAMoE(dsl) & 25.9 & {\bf 46.1} & 53.7 & 54.4\\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
% table end

% table begin
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{The results on AVACap}
\label{table:activity}
\begin{tabular}{lcccc}
\hline\noalign{\smallskip}
Model & R1 & R5 & R10 & MeanR\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
CLIP4Clip & 40.5 & 73.4 & - & 7.5\\
Ours & {\bf 41.0} & {\bf 73.6} &  {\bf 84.5} & 8.6\\
CAMoE(dsl) & 51.0 & 77.1 & 87.6 & 6.3\\
Ours(dsl) & 48.4 & 77.3 & 86.1 & 8.4\\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
% table end

% table begin
\begin{table*}
	\begin{center}
	\caption{Retrieval results on VATEX. }
	\label{VATEXTable}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{c|ccccc|ccccc} % 控制表格的格式
	\hline
    \multicolumn{3}{c}{}\multicolumn{4}{c}{Text \Longrightarrow Video} &\multicolumn{4}{c}{Video \Longrightarrow Text} \\
    \hline
	Method & R@1 & R@5 & R@10 & MdR & MnR & R@1 & R@5 & R@10 & MdR & MnR \\
    \hline
    Random Baseline                               & 0.2  & 0.7  & 1.05    & 2000.5 & -   & 0.02 & 0.1 & 1.02 & 2100.5 & -\\
    VSE \cite{kiros2014unifying}                  & 28.0 & 64.3 & 76.9    & 3.0    & -   & -    &    - & -    &   -   & - \\
    VSE++ \cite{faghri2017vse++}                  & 33.7 & 70.1 & 81.0    & 2.0    & -   & -    &    - & -    &   -   & - \\
    Dual Enc. \cite{dong2019dual}                 & 31.1 & 67.5 & 78.9    & 3.0    & -   & -    &    - & -    &   -   & - \\
    HGR   \cite{chen2020fine}                     & 35.1 & 73.5 & 83.5    & 2.0    & -   & -    &    - & -    &   -   & - \\
    CLIP \cite{portillo2021straightforward}       & 39.7 & 72.3 & 82.2    & 2.0    & 12.8& 52.7 & 88.8 & 94.9 & 1.0   & 3.8 \\
    SUPPORT-SET \cite{patrick2020support}         & 44.9 & 82.1 & 89.7    & 1.0    & -   & 58.4 & 84.4 & 91.0 & 1.0   & - \\
    CLIP4Clip-seqTransf \cite{luo2021clip4clip}   & 55.9 & 89.2 & 95.0 & 1.0 & 3.9 & 73.2 & 97.1 & 99.1 & 1.0 & 1.7 \\
    CLIP2Video \cite{fang2021clip2video}          & 57.3 & 90.0 & 95.5 & 1.0 & 3.6 & 76.0 & 97.7 & 99.9 & 1.0 & 1.5 \\
	\hline
	\textbf{Ours} & \textbf{59.1} & \textbf{90.0} & \textbf{95.2} & \textbf{1.0}  & \textbf{3.5} & \textbf{75.1}	& \textbf{97.0} &	\textbf{98.8}	& \textbf{1.0} & \textbf{1.7} \\
	
	\hline
		\end{tabular}}
	\end{center}
		\vspace{-0.4cm}
\end{table*}

\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{The results on DiDeMo}
\label{table:didemo}
\begin{tabular}{lcccc}
\hline\noalign{\smallskip}
Model & R1 & R5 & R10 & MeanR\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
CLIP4Clip & 43.4 & 70.2 & 80.6 & 17.5\\
QB-Norm & 43.5 & 71.4 & 80.9 & -\\
Ours & 41.8 & {\bf 71.6} &  {\bf 82.0} & 14.8\\
CAMoE(dsl) & 43.8 & 71.4 & 79.9 & 16.3\\
Ours(dsl) & 47.4 & 73.6 & 82.4 & 12.9\\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
% table end


\subsection{Comparison with other Video Encoder.}
Previous work such as ViViT\cite{arnab2021vivit}, TimeSformer\cite{bertasius2021space} and NIPs2021napian have explored many forms of video ViT. We compare complexity with other video ViT in table \ref{table:vivitcomplexity}. 

% table begin
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Complex of our video encoder and other Video ViT. Suppose we have video of T frames and N tokens per frame. K means selecting K tokens per frame in TimeSformer's L+G strategy. We refer readers to TimeSformer\cite{bertasius2021space} and ViViT\cite{arnab2021vivit} to know details about aggregation strategy}
\label{table:vivitcomplexity}
\begin{tabular}{l|c|l}
\hline\noalign{\smallskip}
Model & Aggregation Strategy & Time Complexity \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
ViT & - & $O$(N^2) \\
TimeSformer\cite{bertasius2021space} & ST &  $O$((TN)^2) \\
TimeSformer\cite{bertasius2021space} & T+S &  $O$(N^2 + T^2) \\
TimeSformer\cite{bertasius2021space} & L+G &  $O$((TK)^2) \\
ViViT\cite{arnab2021vivit} & Factorised Encoder &  $O$(N^2 + T^2) \\
ViViT\cite{arnab2021vivit} & Factorised Self-Attention &  $O$(N^2 + T^2) \\
ViViT\cite{arnab2021vivit} & Factorised dot-product &  $O$(N^2 + T^2) \\
Ours & - &  $O$(N^2 + T^2) \\

\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
% table end
